Mixed LICORS: A Nonparametric Algorithm for Predictive State Reconstruction

We introduce 'mixed LICORS', an algorithm for learning nonlinear, high-dimensional dynamics from spatio-temporal data, suitable for both prediction and simulation. Mixed LICORS extends the recent LICORS algorithm (Goerg and Shalizi, 2012) from hard clustering of predictive distributions to a non-parametric, EM-like soft clustering. This retains the asymptotic predictive optimality of LICORS, but, as we show in simulations, greatly improves out-of-sample forecasts with limited data. The new method is implemented in the publicly-available R package "LICORS" (http://cran.r-project.org/web/packages/LICORS/).

==> arxiv_load_packages.tex <==
%\usepackage{float}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
%\usepackage{lineno} 

\usepackage{amssymb, amsmath, amscd}



\usepackage{graphicx}
\usepackage{amsthm}
\usepackage{verbatim}
%\usepackage{subfig}
%\usepackage{epstopdf}

\usepackage{algorithm}
\usepackage[noend]{algorithmic}
%\usepackage{diagxy}
\usepackage{tikz}
\usetikzlibrary{shapes,arrows, fadings, calc, positioning}

%\usepackage{fancyhdr}
%\usepackage{setspace}
\usepackage{url}
%\usepackage{enumitem}
\usepackage{enumerate}

\usepackage{paralist} % for inline list; e.g. here i) is this and ii) that (no line break)
\usepackage{caption}
\DeclareCaptionType{copyrightbox}
\usepackage{subcaption}
